Machine Learning on Graphs: A Model and Comprehensive Taxonomy

There has been a surge of recent interest in learning representations for graph-structured data. Graph representation learning methods have generally fallen into three main categories, based on the availability of labeled data. The first, network embedding (such as shallow graph embedding or graph auto-encoders), focuses on learning unsupervised representations of relational structure. The second, graph regularized neural networks, leverages graphs to augment neural network losses with a regularization objective for semi-supervised learning. The third, graph neural networks, aims to learn differentiable functions over discrete topologies with arbitrary structure. However, despite the popularity of these areas there has been surprisingly little work on unifying the three paradigms. Here, we aim to bridge the gap between graph neural networks, network embedding and graph regularization models. We propose a comprehensive taxonomy of representation learning methods for graph-structured data, aiming to unify several disparate bodies of work. Specifically, we propose a Graph Encoder Decoder Model (GRAPHEDM), which generalizes popular algorithms for semi-supervised learning on graphs (e.g. GraphSage, Graph Convolutional Networks, Graph Attention Networks), and unsupervised learning of graph representations (e.g. DeepWalk, node2vec, etc) into a single consistent approach. To illustrate the generality of this approach, we fit over thirty existing methods into this framework. We believe that this unifying view both provides a solid foundation for understanding the intuition behind these methods, and enables future research in the area.

==> 02non_euclidean.tex <==
\input{figures/non_euclidean.tex}
% Successes of CNNs
Convolutional Neural Networks (CNNs) have achieved unprecedented performance in pattern recognition tasks such as image classification or speech recognition. 
These major successes have been restricted to particular types of data that have a simple
relational structure (e.g. sequential data, or data following regular patterns). 
For instance, images can be viewed as Euclidean data discretized on 2D regular grids, while text data follows a simple sequential structure. 
In other words, most common deep learning models usually assume that the data has an underlying Euclidean structure and leverage its inherent properties such as its linear structure and useful operators including inner products and additions. 

% Generalize CNNs to graphs is not trivial
However, non-Euclidean data such as graphs arise in many important applications including social networks, biology or computer vision. 
In particular, operations like convolutions cannot be directly applied on irregular graph domains. For instance in images, each pixel has the same neighborhood structure, allowing to apply the same filter weights at multiple locations in the image. 
However in graphs, one can’t define an ordering of node since each node might have a different neighborhood structure~(\cref{fig:non_euclidean_vs_euclidean}). 
Furthermore, Euclidean convolutions strongly rely on geometric priors such as shift invariance. 
Such priors lead to significant improvements in computational cost and model complexity, but can’t be leveraged when the data is defined on a non-Euclidean domain: translations might not even be defined on non-Euclidean domains.

% GDL
This led to the development of Geometric Deep Learning (GDL) research which aims at applying deep learning techniques to non-Euclidean data. 
Broadly speaking, GDL refers to methods applying deep learning to graphs or manifolds. 
In this survey we focus specifically on graph representation learning methods and refer the reader to the GDL survey by \citet{bronstein2017geometric} for more details about learning on manifolds.
Note that some of the methods we cover in this survey can also be applied to manifolds: the first step is to build a discrete graph structure using the manifold geometry, and then apply graph embedding methods. 

% Unsupervised GRL
As described by \citet{bronstein2017geometric} in their review paper, GDL can be divided into two classes of learning problems. 
The first family of problems aims at \textbf{characterizing the structure of a non-Euclidean domain}.
At a high level, the goal in this family of problems is to learn some low-dimensional embedding space that preserves the geometry of high-dimensional non-Euclidean input data. 
Methods commonly known as \textit{manifold learning} fall under this category and we will review some linear and non-linear dimensionality reduction techniques in~\cref{subsec:laplacian_unsup_shallow}. 
More recently, there has been attempts to apply techniques employed for word embeddings, known as skip-gram, to learn graph embeddings~(\cref{subsec:skip_gram_unsup}).

% Supervised GRL
The second family of problems aims at \textbf{analyzing data defined on a non-Euclidean domain}. 
In this scenario, the input data is presented as signals defined on a graph or manifold, and the goal is to analyze those signals and extract meaningful information, usually for a downstream classification task.
This is the supervised graph embedding setting, and we review the differences between supervised and unsupervised embeddings in~\cref{subsec:supervision}.
When the data is defined on a graphs, the signals are commonly referred to as node features and we discuss their role in~\cref{subsec:node_features}.
Note that the underlying graph domain might be fixed, which is the \textbf{transductive} learning setting, but can also vary in the \textbf{inductive} learning setting. 
We review the differences between transductive and inductive learning in~\cref{subsec:inductive_transductive}. 

% Non-Euclidean embedding space
Finally, note that both families of problems mentioned so far aim at learning low-dimensional Euclidean embedding spaces. 
Recently, there has been interest for \textbf{non-Euclidean representation learning} methods, which aim at learning non-Euclidean embedding spaces such as hyperbolic or spherical spaces.
The main motivations for this body of work is to use a \textbf{continuous embedding space that resembles the underlying discrete structure of the input data} it tries to embed. 
For instance, the hyperbolic space is a continuous version of trees and can embed tree-like structure with lower distortion than Euclidean embedding spaces \cite{sarkar2011low,de2018representation}. 
Similar to the two types of problems above, there have been works trying to characterize the structure of graphs using non-Euclidean embeddings~(\cref{subsec:non_euclidean_unsup}), while other works analyze data defined on graphs using non-Euclidean embeddings~(\cref{subsec:non_euclidean_sup}). 
%

==> figures/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> figures/latex_tree_hierarchy.tex <==
\forestset{
  L1/.style={rectangle, draw, fill=blue!20!red!20, rounded corners, thick,edge={line width=0.5pt}},
  L2/.style={rectangle, draw, fill=blue!20!green!20, rounded corners, thick,edge={line width=0.5pt}},
  L3/.style={rectangle, draw, fill=gray!20, rounded corners, thick,edge={line width=0.5pt}},
  L4/.style={rectangle, draw, fill=blue!15, rounded corners, thick,edge={line width=0.5pt}},
  L5/.style={rectangle, draw, fill=yellow!20, rounded corners, thick,edge={line width=0.5pt}},
  %%%%%%%%%%%%%
}
\hspace{2in}
\begin{minipage}[t]{\textwidth}
    \vspace{0.2cm}
    {\large \textbf{Legend}}
    \\
    \begin{forest}
        for tree={
            align=center, % allow multiple lines
            grow=0,reversed, % tree direction
            parent anchor=east,child anchor=west, % edge anchors
            edge={line cap=round},outer sep=+1pt, % edge/node connection
            rounded corners,minimum width=15mm,minimum height=8mm, % node shape
            l sep=2mm % level distance
        }
        [Shallow embeddings,L1]
    \end{forest}
    \\
    \begin{forest}
        for tree={
            align=center, % allow multiple lines
            grow=0,reversed, % tree direction
            parent anchor=east,child anchor=west, % edge anchors
            edge={line cap=round},outer sep=+1pt, % edge/node connection
            rounded corners,minimum width=15mm,minimum height=8mm, % node shape
            l sep=5mm % level distance
        }
        [Auto-encoders,L5]
    \end{forest}
    \\
    \begin{forest}
        for tree={
            align=center, % allow multiple lines
            grow=0,reversed, % tree direction
            parent anchor=east,child anchor=west, % edge anchors
            edge={line cap=round},outer sep=+1pt, % edge/node connection
            rounded corners,minimum width=15mm,minimum height=8mm, % node shape
            l sep=5mm % level distance
        }
        [Graph regularization,L4]
    \end{forest}
    \\  
    \begin{forest}
        for tree={
            align=center, % allow multiple lines
            grow=0,reversed, % tree direction
            parent anchor=east,child anchor=west, % edge anchors
            edge={line cap=round},outer sep=+1pt, % edge/node connection
            rounded corners,minimum width=15mm,minimum height=8mm, % node shape
            l sep=5mm % level distance
        }
        [Graph neural networks,L2]
    \end{forest}
    \\
    \vspace{-3in}
\end{minipage} % end legend
\\
%\fbox{
\begin{forest}
    for tree={
        align=center, % allow multiple lines
        grow=0,reversed, % tree direction
        parent anchor=east,child anchor=west, % edge anchors
        edge={line cap=round},outer sep=+1pt, % edge/node connection
        rounded corners,minimum width=15mm,minimum height=8mm, % node shape
        l sep=3mm % level distance
    }
    [\textbf{Graph} \\
    \textbf{Embedding},L3
        [\textbf{Unsupervised}\\ $(\alpha \eqtext 0)$\\{\hyperref[sec:unsup_models]{Section \ref{sec:unsup_models}}},L3
            [$X \eqtext I$,L3
                [ENC$(\Theta^E)$,L1
                    [\textbf{Laplacian} \\  {\hyperref[subsec:laplacian_unsup_shallow]{Section \ref{subsec:laplacian_unsup_shallow}}},L1
                        [
                            MDS \cite{kruskal1964multidimensional} \\
                            IsoMAP \cite{tenenbaum2000global} \\
                            LLE \cite{roweis2000nonlinear} 
                            LE \cite{belkin2002laplacian},L1
                        ]
                    ]
                    [\textbf{Non-Euclidean}\\ {\hyperref[subsec:non_euclidean_unsup]{Section \ref{subsec:non_euclidean_unsup}}},L1
                        [
                            Poincar\'e  \cite{nickel2017poincare} \\
                            Lorentz \cite{nickel2018learning} \\
                            Product \cite{gu2018learning},L1
                        ]
                    ]
                    [\textbf{Matrix}\\ \textbf{Factorization} \\ {\hyperref[subsec:matrix]{Section \ref{subsec:matrix}}},L1
                        [
                            GF \cite{ahmed2013distributed} \\
                            GraRep \cite{cao2015grarep}\\
                            HOPE \cite{ou2016asymmetric},L1
                        ]
                    ]
                    [\textbf{Skip-gram} \\ {\hyperref[subsec:skip_gram_unsup]{Section \ref{subsec:skip_gram_unsup}}},L1
                        [
                            DeepWalk \cite{perozzi2014deepwalk} \\
                            node2vec \cite{grover2016node2vec}\\
                            WYS \cite{abu2017watch}  LINE \cite{tang2015line} \\
                            HARP \cite{chen2017harp},L1
                        ]   
                    ]
                ]
                [ENC$(W; \Theta^E)$,L5
                    [\textbf{Autoencoders} \\ {\hyperref[subsec:auto_enc]{Section \ref{subsec:auto_enc}}},L5
                        [
                            SDNE \cite{wang2016structural} \\
                            DNGR \cite{cao2016deep},L5
                        ]
                    ]
                ]
            ]
            [$X \neq I$,L3
                [ENC$(W\comma X ; \Theta^E)$,L2
                    [\textbf{Spectral}  \\ {\hyperref[subsec:neighbour_unsup]{Section \ref{subsec:neighbour_unsup}}},L2
                        [GAE \cite{kipf2016variational}\\ 
                        Graphite \cite{grover2018graphite},L2]
                    ]
                ]
            ]        
        ]
        [\textbf{Supervised} \\ $(\alpha \neq 0)$\\ {\hyperref[sec:sup_models]{Section \ref{sec:sup_models}}},L3
            [$X \eqtext I$,L3
                [ENC$(\Theta^E)$,L1
                    [\textbf{Laplacian}  \\ {\hyperref[subsec:shallow_sup]{Section \ref{subsec:shallow_sup}}},L1
                        [
                            LP \cite{zhu2002learning} \\
                            Consistency \cite{zhou2004learning},L1
                        ]
                    ]
                ]
            ]
            [$X \neq I$,L3
                [ENC$(X ; \Theta^E)$,L4
                    [\textbf{Laplacian}  \\ {\hyperref[subsubsec:laplacian_reg_sup]{Section \ref{subsubsec:laplacian_reg_sup}}},L4
                        [
                            ManiReg \cite{belkin2006manifold} \\
                            SemiEmbed \cite{weston2012deep} NGM \cite{bui2017neural},L4
                        ]
                    ]
                     [\textbf{Skip-gram}  \\ {\hyperref[subsubsec:skip_gram_sup]{Section \ref{subsubsec:skip_gram_sup}}},L4
                        [Planetoid \cite{yang2016revisiting},L4]
                    ]
                ]
                [ENC$(W\comma X ; \Theta^E)$,L2
                    [\textbf{Message passing}  \\ {\hyperref[subsec:gnn_sup]{Section \ref{subsec:gnn_sup}}},L2
                        [
                            GNN \cite{scarselli2009graph} GGSNNs \cite{li2015gated} \\
                            MPNN \cite{gilmer2017neural} GraphNets \cite{battaglia2016interaction},L2
                        ]
                    ]
                    [\textbf{Spectral}  \\ {\hyperref[subsec:spectral]{Section \ref{subsec:spectral}}},L2
                        [
                            SCNN \cite{bruna2013spectral,henaff2015deep} \\
                            ChebyNet \cite{defferrard2016convolutional} GCN \cite{kipf2016semi},L2
                            %SGC \cite{wu2019simplifying} 
                        ]
                    ]
                    [\textbf{Spatial}  \\ {\hyperref[subsec:spatial]{Section \ref{subsec:spatial}}},L2
                        [
                            SAGE \cite{hamilton2017inductive} \\
                            MoNet \cite{monti2017geometric} GAT \cite{velickovic2017graph},L2
                        ]
                    ]
                    [\textbf{Non-Euclidean} \\ {\hyperref[subsec:non_euclidean_sup]{Section \ref{subsec:non_euclidean_sup}}},L2
                        [
                            HGCN \cite{chami2019hyperbolic} \\
                            HGNN \cite{liu2019hyperbolic},L2
                        ]
                    ]
                ]
            ]
        ]
    ]   
\end{forest}
%} 
